A Light Touch for Heavily Constrained SGD

Minimizing empirical risk subject to a set of constraints can be a useful strategy for learning restricted classes of functions, such as monotonic functions, submodular functions, classifiers that guarantee a certain class label for some subset of examples, etc. However, these restrictions may result in a very large number of constraints. Projected stochastic gradient descent (SGD) is often the default choice for large-scale optimization in machine learning, but requires a projection after each update. For heavily-constrained objectives, we propose an efficient extension of SGD that stays close to the feasible region while only applying constraints probabilistically at each iteration. Theoretical analysis shows a compelling trade-off between per-iteration work and the number of iterations needed on problems with a large number of constraints.

==> Makefile <==
LATEX = latex
PDFLATEX = pdflatex -file-line-error -halt-on-error
PS2PDF = ps2pdf

SPELLCHECK_FILES = $(wildcard main.tex abstract.tex sec-*.tex app-*.tex figures/*.tex theorems/*.tex)
TEX_FILES = $(wildcard *.tex */*.tex)
EPS_IMAGES = $(wildcard images/*.eps)
FILES = $(TEX_FILES) $(EPS_IMAGES)

BEGIN_PAGE_COMMAND = cat main.aux | sed -n 's/\\\newlabel{document:begin}{{[^}]*}{\([^}]*\)}{[^}]*}{[^}]*}{[^}]*}}/\1/p'
MIDDLE_PAGE_COMMAND = cat main.aux | sed -n 's/\\\newlabel{document:middle}{{[^}]*}{\([^}]*\)}{[^}]*}{[^}]*}{[^}]*}}/\1/p'
APPENDIX_PAGE_COMMAND = cat main.aux | sed -n 's/\\\newlabel{document:appendix}{{[^}]*}{\([^}]*\)}{[^}]*}{[^}]*}{[^}]*}}/\1/p'
END_PAGE_COMMAND = cat main.aux | sed -n 's/\\\newlabel{document:end}{{[^}]*}{\([^}]*\)}{[^}]*}{[^}]*}{[^}]*}}/\1/p'

.PHONY : all
#all: main.pdf light_touch.pdf light_touch_supplementary_material.pdf
all: main.pdf

%.bbl: %.bib $(FILES)
	$(MAKE) -C images
	$(PDFLATEX) ${basename $<}
	$(PDFLATEX) ${basename $<}
	bibtex ${basename $<}

%.pdf: %.tex %.bbl $(FILES)
	$(MAKE) -C images
	$(PDFLATEX) ${basename $<}
	$(PDFLATEX) ${basename $<}
	$(PDFLATEX) ${basename $<}

light_touch.pdf: main.pdf
	pdftk main.pdf cat `$(BEGIN_PAGE_COMMAND)`-`$(MIDDLE_PAGE_COMMAND)` output light_touch.pdf

light_touch_supplementary_material.pdf: main.pdf
	pdftk main.pdf cat `$(APPENDIX_PAGE_COMMAND)`-`$(END_PAGE_COMMAND)` output light_touch_supplementary_material.pdf

dictionary.txt: words.txt main.bib $(SPELLCHECK_FILES)
	cp words.txt dictionary.txt
	cat main.bib | sed -n "s/^@[^{]*{//p" | sed "s/[[:digit:]]*,[[:space:]]*$$//" | sort | uniq >> dictionary.txt
	#cat $(SPELLCHECK_FILES) | sed -n "s/^.*\\label{\([^}]*\)}.*$$/\1/p" | sed "s/[:-]/\n/g" | sort | uniq >> dictionary.txt

dictionary.rws: dictionary.txt
	aspell --lang=en create master ./$@ < $<

spellcheck: dictionary.rws $(SPELLCHECK_FILES)
	for ii in $(SPELLCHECK_FILES) ; do aspell -d en_US --extra-dicts=`pwd`/dictionary.rws -c $$ii ; done

.PHONY: clean
clean:
	$(MAKE) -C images clean
	rm -f dictionary.txt dictionary.rws
	rm -f main.log main.aux main.bbl main.blg main.out
	rm -f main.pdf light_touch.pdf light_touch_supplementary_material.pdf


==> app-ordering.tex <==
\section{Projecting onto Ordering Constraints}\label{sec:ordering}

\input{figures/alg-ordering}
%
Consider the problem of projecting a vector $\tilde{w} \in \R^d$ onto the
ordering constraints of \appref{constraints:gamma} \wrt the Euclidean norm:
%
\begin{align*}
  %
  \min_{w} & \norm{w - \tilde{w}}_2^2 \\
  %
  \subjectto & w_i \le w_{i + 1} \;\; \forall i \in \left\{1, \dots, d -
  1\right\} \eqperiod
  %
\end{align*}
%
It follows from the KKT conditions that there exist $\lambda_i \ge 0$ for which
$w_i = \tilde{w}_i + \lambda_{i-1} - \lambda_i$. Hence, if $\lambda_{l-1} =
\lambda_{u+1} = 0$ and $\lambda_i > 0$ for $l \le k \le u$, summation yields:
%
\begin{equation*}
  %
  \sum_{i=l}^u w_i
  %
  = \sum_{i=l}^u \tilde{w}_i + \lambda_{l-1} - \lambda_{u+1}
  %
  = \sum_{i=l}^u \tilde{w}_i \eqperiod
  %
\end{equation*}
%
Combined with the complementary slackness property that $\lambda_i (w_i -
w_{i+1}) = 0$, this shows that along every ``chain'' of active constraints,
$w_i = (\sum_{i=l}^u \tilde{w}_i) / (u - l + 1)$, \ie the optimum value is the
average value of $\tilde{w}_i$ along the chain.

This immediately suggests that a projection algorithm could be based on
identifying those elements which are connected via active constraints,
and then averaging over them. Indeed, we can do exactly this, by initially
identifying each element $w_i$ with a cluster, and then iteratively finding
violated constraints, and merging the two involved clusters. Because,
in order for a constraint to be violated, the ``left'' cluster must be
larger than the ``right'' one, it follows that merging them will reduce the
values on the left cluster, and increase those of the right, showing that
no formerly-active constraints can become inactive due to the two clusters
being merged, so we can consider violated constraints in any order we choose.

\algref{ordering} contains this algorithm. In lines 9-13 it finds a violated
constraint, and merges the two involved clusters, after which two new
constraints (those on each ``end'' of the new cluster) could be violated, and
must be checked (lines 14-25).

Using a disjoint-set data structure $\disjointsets$ to represent the
clusters~\citep{WikipediaDisjointSet} results in each $\mbox{Find}$ and
$\mbox{Union}$ operation taking amortized $O(\alpha(d))$ time, where $\alpha$
is the inverse Ackermann function. Representing the set of violated constraints
$\violations$ as a doubly linked list of constraint indices, with an associated
size-$d$ array where the $i$th element contains a pointer to the associated
list element if $i \in \violations$, and \nullptr otherwise, reduces all
operations on $\violations$ to constant time.

We require $O(n)$ initialization and cleanup time (lines 1-7 and 26-28), and
the main loop can iterate at most $d-1$ times (once per constraint), so the
overall runtime required to perform the projection is $O(d \alpha(d))$.
%
In terms of the number of constraint checks: $d-1$ constraints are checked on
line 7, and at most two constraints are checked every time we go through the
main loop, so there are $O(d)$ constraint evaluations.


==> figures/alg-ordering.tex <==
\newcommand{\disjointsets}{\mathcal{S}}
\newcommand{\violations}{\mathcal{V}}
\newcommand{\numerators}{N}
\newcommand{\denominators}{D}
\newcommand{\lowers}{L}
\newcommand{\uppers}{U}

\begin{algorithm*}[t]

\begin{pseudocode}
%
%\codename \textbf{\orderingname} \\
%
\codeline Initialize $\disjointsets$ as disjoint-set data structure with sets $1, \dots, d$\\
\codeline Initialize $\numerators = w$, $\denominators = \mathbf{1}$ \codecomment{numerators and denominators of elements of $\disjointsets$}\\
\codeline Initialize $\lowers = [1,\dots,d]^T$, $\uppers = [1,\dots,d]^T$ \codecomment{lower and upper indices of elements of $\disjointsets$}\\
\codeline Initialize $\violations = \emptyset$ \codecomment{set of violated constraints}\\
\codeline For $i = 1$ to $d - 1$: \codecomment{find all violated constraints} \\
\codeline \>If $w_i > w_{i+1}$:\\
\codeline \>\>Insert $i$ into $\violations$ \codecomment{$i \in \mathcal{V}$ means $w_i > w_{i+1}$}\\
\codeline While $\violations$ is nonempty: \codecomment{as long as any constraints are violated} \\
\codeline \>Choose $i \in \violations$ arbitrarily, and erase $i$ from $\violations$\\
\codeline \>Let $k_{<} = \mbox{Find}(\disjointsets, i)$, $k_{>} = \mbox{Find}(\disjointsets, i+1)$\\
\codeline \>Let $k = \mbox{Union}(\disjointsets, i, i+1)$\\
\codeline \>Set $\numerators_k = \numerators_{k_{<}} + \numerators_{k_{>}}$, $\denominators_k = \denominators_{k_{<}} + \denominators_{k_{>}}$\\
\codeline \>Set $\lowers_k = \lowers_{k_{<}}$, $\uppers_k = \uppers_{k_{>}}$\\
\codeline \>If $\lowers_k > 1$: \codecomment{do we need to check if $w_{\lowers_k - 1} \le w_{\lowers_k}$?}\\
\codeline \>\>Let $k_{<} = \mbox{Find}(\disjointsets, \lowers_k - 1)$\\
\codeline \>\>If $\numerators_{k_{<}} / \denominators_{k_{<}} > \numerators_k / \denominators_k$:\\
\codeline \>\>\>Insert $\lowers_k - 1$ into $\violations$, if absent\\
\codeline \>\>Else:\\
\codeline \>\>\>Erase $\lowers_k - 1$ from $\violations$, if present\\
\codeline \>If $\uppers_k < d$: \codecomment{do we need to check if $w_{\uppers_k} \le w_{\uppers_k + 1}$?} \\
\codeline \>\>Let $k_{>} = \mbox{Find}(\disjointsets, \uppers_k + 1)$\\
\codeline \>\>If $\numerators_{k} / \denominators_{k} > \numerators_{k_{>}} / \denominators_{k_{>}}$:\\
\codeline \>\>\>Insert $\uppers_k$ into $\violations$, if absent\\
\codeline \>\>Else:\\
\codeline \>\>\>Erase $\uppers_k$ from $\violations$, if present\\
\codeline For $i = 1$ to $d - 1$: \codecomment{set $w_i$ to the average over the $\disjointsets$-element containing it}\\
\codeline \>Let $k = \mbox{Find}(\disjointsets, i)$\\
\codeline \>Set $w_i = \numerators_k / \denominators_k$\\
\codeline Return $w$
%
\end{pseudocode}

\caption{
  %
  \textbf{(\orderingname)} Projects onto ordering constraints
  (\appref{constraints:gamma}) \wrt the Euclidean norm. As discussed in
  \appref{ordering}, this algorithm evaluates $O(d)$ constraints, and has a
  runtime bound of $O(d \alpha(d))$, where $\alpha$ is the inverse Ackermann
  function.
  %
}

\label{alg:ordering}

\end{algorithm*}

